Monocular Depth Estimation for Soft Visuotactile Sensors

Fluid-filled soft visuotactile sensors such as the Soft-bubbles alleviate key challenges for robust manipulation, as they enable reliable grasps along with the ability to obtain high-resolution sensory feedback on contact geometry and forces. Although they are simple in construction, their utility has been limited due to size constraints introduced by enclosed custom IR/depth imaging sensors to directly measure surface deformations. Towards mitigating this limitation, we investigate the application of state-of-the-art monocular depth estimation to infer dense internal (tactile) depth maps directly from the internal single small IR imaging sensor. Through real-world experiments, we show that deep networks typically used for long-range depth estimation (1-100m) can be effectively trained for precise predictions at a much shorter range (1-100mm) inside a mostly textureless deformable fluid-filled sensor. We propose a simple supervised learning process to train an object-agnostic network requiring less than 10 random poses in contact for less than 10 seconds for a small set of diverse objects (mug, wine glass, box, and fingers in our experiments). We show that our approach is sample-efficient, accurate, and generalizes across different objects and sensor configurations unseen at training time. Finally, we discuss the implications of our approach for the design of soft visuotactile sensors and grippers.

==> sections/depth_temp.tex <==
% CROSS-OBJECT GENERALIZATION (BTS)

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{BTS: Cross-object generalization (dotted)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{LOO}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Mug}}}}

& \textit{Mug}
& 0.041 & 0.016 & 0.053 & 4.859 & 0.712 & 0.924 & 0.977 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Glass}}}}

& \textit{Mug}
& 0.017 & 0.008 & 0.024 & 2.292 & 0.954 & 0.996 & 0.999 \\
& \textit{Box}
& 0.017 & 0.008 & 0.024 & 2.305 & 0.953 & 0.995 & 0.999 \\
& \textit{Glass}
& 0.034 & 0.013 & 0.045 & 4.078 & 0.775 & 0.950 & 0.987 \\
& \textit{Fingers}
& 0.018 & 0.008 & 0.024 & 2.353 & 0.949 & 0.995 & 0.999 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Fingers}}}}

& \textit{Mug}
& 0.019 & 0.008 & 0.025 & 2.336 & 0.947 & 0.996 & 0.999 \\
& \textit{Box}
& 0.019 & 0.008 & 0.025 & 2.349 & 0.945 & 0.995 & 0.999 \\
& \textit{Glass}
& 0.019 & 0.008 & 0.025 & 2.295 & 0.949 & 0.995 & 0.999 \\
& \textit{Fingers}
& 0.037 & 0.017 & 0.053 & 5.273 & 0.776 & 0.925 & 0.968 \\


\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Box}}}}

& \textit{Mug}
& 0.018 & 0.008 & 0.025 & 2.431 & 0.948 & 0.994 & 0.999\\
& \textit{Box}
& 0.043 & 0.017 & 0.056 & 5.273 & 0.721 & 0.882 & 0.952 \\
& \textit{Glass}
& 0.017 & 0.008 & 0.024 & 2.372 & 0.952 & 0.994 & 0.999 \\
& \textit{Fingers}
& 0.018 & 0.008 & 0.025 & 2.475 & 0.945 & 0.993 & 0.999 \\

\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (BTS \cite{lee2019big}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-obj-dotted}
\end{table*}

% DOTLESS CROSS-OBJECT GENERALIZATION

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{PackNet: Cross-object generalization (dotless)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{LOO}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Glass}}}}

& \textit{Glass}
& 0.033 & 0.022 & 0.040 & 3.962 & 0.778 & 0.957 & 0.997 \\
& \textit{Box}
& 0.009 & 0.006 & 0.011 & 1.016 & 0.998 & 1.000 & 1.000 \\
& \textit{Fingers}
& 0.010 & 0.008 & 0.014 & 1.325 & 0.992 & 0.999 & 1.000 \\

\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Box}}}}

& \textit{Glass}
& 0.008 & 0.007 & 0.012 & 1.206 & 0.994 & 0.999 & 0.999 \\
& \textit{Box}
& 0.030 & 0.021 & 0.038 & 3.193 & 0.791 & 0.971 & 0.999 \\
& \textit{Fingers}
& 0.009 & 0.007 & 0.014 & 1.314 & 0.992 & 0.999 & 1.000 \\

\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Fingers}}}}

& \textit{Glass}
& 0.008 & 0.006 & 0.011 & 1.052 & 0.997 & 1.000 & 1.000 \\
& \textit{Box}
& 0.008 & 0.006 & 0.010 & 1.006 & 0.998 & 1.000 & 1.000 \\
& \textit{Fingers}
& 0.037 & 0.027 & 0.048 & 4.562 & 0.723 & 0.910 & 0.975 \\


\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (PackNet \cite{packnet}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-obj-dotless}
\end{table*}

% CROSS-CAMERA GENERALIZATION

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{PackNet: Cross-camera generalization (dotted)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{Cam}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Left}}}}
& \textit{Mug}
& 0.032 & 0.013 & 0.042 & 3.926 & 0.785 & 0.974 & 0.996 \\
& \textit{Box}
& 0.053 & 0.023 & 0.067 & 5.434 & 0.532 & 0.844 & 0.961 \\
& \textit{Glass}
& 0.064 & 0.028 & 0.080 & 4.738 & 0.377 & 0.780 & 0.949 \\
& \textit{Fingers}
& 0.062 & 0.025 & 0.076 & 6.157 & 0.430 & 0.806 & 0.945 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Right}}}}

& \textit{Mug}
& 0.036 & 0.017 & 0.055 & 4.959 & 0.746 & 0.965 & 0.985 \\
& \textit{Box}
& 0.033 & 0.015 & 0.052 & 5.087 & 0.814 & 0.968 & 0.986 \\
& \textit{Glass}
& 0.048 & 0.021 & 0.068 & 6.246 & 0.602 & 0.918 & 0.974 \\
& \textit{Fingers}
& 0.049 & 0.020 & 0.069 & 6.212 & 0.626 & 0.905 & 0.970 \\

\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (PackNet \cite{packnet}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-cam-dotted}
\end{table*}





==> sections/figure_training.tex <==
\begin{figure*}[t!]
\centering
\subfloat{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/box_rgb_19.png}
} \hspace{-2mm}
\subfloat{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/box_inv_depth_0.png}
} \hspace{-2mm}
\subfloat{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/box_inv_depth_1.png}
} \hspace{-2mm}
\subfloat{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/box_inv_depth_5.png}
} \hspace{-2mm}
\subfloat{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/box_inv_depth_19.png}
\label{fig:dotless_pred}
} \hspace{-2mm}
\subfloat{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/box_depth_19.png}
}
\vspace{-2mm}
\\
\setcounter{subfigure}{0}
\subfloat[Input image]{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/finger_rgb_19.png}
} \hspace{-2mm}
\subfloat[Epoch 5]{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/finger_inv_depth_0.png}
} \hspace{-2mm}
\subfloat[Epoch 20]{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/finger_inv_depth_1.png}
} \hspace{-2mm}
\subfloat[Epoch 50]{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/finger_inv_depth_5.png}
} \hspace{-2mm}
\subfloat[Epoch 100]{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/finger_inv_depth_19.png}
\label{fig:dotless_pred}
} \hspace{-2mm}
\subfloat[Ground-truth]{
\includegraphics[width=0.16\textwidth,height=2cm]{figures/training/finger_depth_19.png}
\label{fig:dotless_pred}
}

\caption{Example of intermediate predicted depth maps, showing the gradual convergence of the \textit{PackNet} depth network during training. In (f), missing areas are due to the sparsity in the ground-truth depth maps, which contains invalid pixels that are masked out (Equation \ref{eq:loss}).}
\label{fig:training-box}
\end{figure*}

==> sections/supp_loo.tex <==

% CROSS-OBJECT GENERALIZATION (PACKNET)

\begin{table*}[h!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.1}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{Out-of-Class Generalization (dotless dataset)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{ResNet}}}}
& \textit{Wine Glass} & 0.033 & 0.025 & 0.044 & \textbf{4.030} & 0.792 & \textbf{0.928} & 0.983 \\
& \textit{Fingers} & \textbf{0.033} & \textbf{0.025} & \textbf{0.042} & \textbf{3.991} & \textbf{0.774} & \textbf{0.955} & \textbf{0.990} \\
& \textit{Box} & 0.039 & 0.030 & 0.051 & 4.234 & 0.722 & 0.900 & 0.984 \\
\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{BTS}}}}
& \textit{Wine Glass} & 0.038 & 0.029 & 0.051 & 4.084 & 0.762 & 0.901 & 0.976 \\
& \textit{Fingers} & 0.038 & 0.028 & 0.049 & 4.057 & 0.733 & 0.912 & 0.988 \\
& \textit{Box} & 0.032 & 0.024 & 0.042 & 4.051 & 0.784 & 0.953 & 0.989 \\
\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{PackNet}}}}
& \textit{Wine Glass} & \textbf{0.031} & \textbf{0.024} & \textbf{0.043} & 4.146 & \textbf{0.810} & 0.925 & \textbf{0.984} \\
& \textit{Fingers} & 0.037 & 0.029 & 0.049 & 4.612 & 0.737 & 0.911 & 0.968 \\
& \textit{Box} & \textbf{0.030} & \textbf{0.022} & \textbf{0.038} & \textbf{3.172} & \textbf{0.807} & \textbf{0.970} & \textbf{0.997} \\
\bottomrule

%\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{ResNet} \cite{godard2018digging2}}}
%& \textit{Mug} & 0.034 & 0.013 & 0.041 & 3.230 & 0.776 & 0.978 & 0.997 \\
%& \textit{Glass} & 0.030 & 0.012 & 0.043 & 3.868 & 0.811 & 0.973 & 0.997 \\
%& \textit{Finger} & 0.028 & 0.014 & 0.046 & 4.352 & 0.845 & 0.972 & 0.990 \\
%& \textit{Box} & 0.042 & 0.017 & 0.056 & 5.244 & 0.702 & 0.907 & 0.966 \\

\end{tabular}
}
\caption{Monocular depth estimation results for cross-dataset generalization using different networks. Independent models trained on 2/3 object datasets plus the no contact dataset, evaluated on the remaining one.}
\label{tab:cross-object}
\end{table*}



==> sections/supp_networks.tex <==

An architectural overview of each depth network considered in this work can be found in Table \ref{tab:networks} (for a more detailed description please refer to~\
\cite{he2016deep,packnet,lee2019big}). Each network receives as input a $224 \times 224$ grayscale image, and outputs a $224 \times 224$ image with per-pixel metric depth estimates.  We also include inference times for each network (batch size of $1$, measured on a Titan V100 GPU card), with \textit{ResNet} achieving the fastest performance, with 58 fps (frames per second); followed by \textit{PackNet}, with 24 fps; and finally \textit{BTS}, with 20 fps. Additionally, we show a high level diagram of the proposed learning framework in Figure~\ref{fig:framework}.

\begin{figure}[h!]
\vspace{5mm}
\includegraphics[width=\linewidth]{figures/bubble_diagram.pdf}
\caption{Diagram of our proposed framework. We use as input a $H \times W$ grayscale image, that is processed by our \textit{Depth Network} to produce an estimated depth map of the same resolution. At training time, the corresponding ground-truth depth map is also provided, and the \textit{Depth Network} is optimized as to minimize the difference between estimated and ground-truth depth maps, given an objective function (Equation 2, main paper). The estimated depth map is lifted to 3D using the camera model, to produce an estimated pointcloud, and can then be used for downstream applications (e.g. pose estimation).}
\label{fig:framework}
\end{figure}


\begin{table*}[!t]%
\small
  \centering
\resizebox{0.49\linewidth}{!}{
\subfloat[ResNet \cite{godard2018digging2} (58  fps)]{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[b]{l|l|c|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\toprule
\multicolumn{5}{c}{\textbf{ResidualBlock (K, S)}} \\ 
\midrule
\#A & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & K & 1 &  \\
\#B & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & K & S &  \\
\toprule
\multicolumn{5}{c}{\textbf{UpsampleBlock (\#skip)}} \\ 
\midrule
\#C & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU$\shortrightarrow$Upsample    & 3 & 1 & \\
\#D & Conv2d ($\#C\oplus\#skip$)$\shortrightarrow$BN$\shortrightarrow$ReLU          & 3 & 1 & \\
\toprule
\toprule
\#0 & Input RGB image & - & - & 3$\times$H$\times$W \\ 
\midrule
\multicolumn{5}{c}{\textbf{Encoder}} \\ \hline
\#1  & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU   & 7 & 1 &  64$\times$H$\times$W \\
\#2  & Max. Pooling                                       & 3 & 2 &  64$\times$H/2$\times$W/2 \\
\#3  & ResidualBlock (x2)                                 & 3 & 2 &  64$\times$H/4$\times$W/4 \\
\#4  & ResidualBlock (x2)                                 & 3 & 2 & 128$\times$H/8$\times$W/8 \\
\#5  & ResidualBlock (x2)                                 & 3 & 2 & 256$\times$H/16$\times$W/16 \\
\#6  & ResidualBlock (x2)                                 & 3 & 2 & 512$\times$H/32$\times$W/32 \\
\midrule
\multicolumn{5}{c}{\textbf{Depth Decoder}} \\ 
\midrule
\#7 & UpsampleBlock (\#5)    & 3 & 1 & 256$\times$H/16$\times$W/16 \\
\#8 & UpsampleBlock (\#4)    & 3 & 1 & 128$\times$H/8$\times$W/8 \\
\#9 & UpsampleBlock (\#3)    & 3 & 1 & 64$\times$H/4$\times$W/4 \\
\#10 & UpsampleBlock (\#2)   & 3 & 1 & 32$\times$H/2$\times$W/2 \\
\#11 & UpsampleBlock (\#1)   & 3 & 1 & 32$\times$H$\times$W \\
\#12 & Conv2d$\shortrightarrow$Sigmoid  & 3 & 1 & 1$\times$H$\times$W \\
\bottomrule
\end{tabular}
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\resizebox{0.49\linewidth}{!}{
\subfloat[PackNet \cite{packnet} (24 fps)]{
\begin{tabular}[b]{l|l|c|c|c}
\toprule
 & \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\midrule
\multicolumn{5}{c}{\textbf{ResidualBlock (K, S)}} \\ \hline
\#A & Conv2d$\shortrightarrow$GN$\shortrightarrow$ELU & K & 1 &  \\
\#B & Conv2d$\shortrightarrow$GN$\shortrightarrow$ELU & K & 1 &  \\
\#C & Conv2d$\shortrightarrow$GN$\shortrightarrow$ELU$\shortrightarrow$Dropout & K & S &  \\
\toprule
\multicolumn{5}{c}{\textbf{UpsampleBlock (\#skip)}} \\ \hline
\#D & Unpacking         & 3 & 1 & \\
\#E & Conv2d ($\#D\oplus\#skip$)$\shortrightarrow$GN$\shortrightarrow$ELU    & 3 & 1 & \\
\toprule
\toprule
\#0 & Input RGB image & - & - & 3$\times$H$\times$W \\ 
\midrule
\multicolumn{5}{c}{\textbf{Encoder}} \\ \hline
\#1 & Conv2d$\shortrightarrow$GN$\shortrightarrow$ELU & 5 & 1 & 64$\times$H$\times$W \\
\#2 & Conv2d$\shortrightarrow$GN$\shortrightarrow$ELU$\shortrightarrow$Packing & 7 & 1 & 64$\times$H$\times$W \\
\#3 & ResidualBlock (x2)$\shortrightarrow$Packing & 3 & 1 & 64$\times$H/4$\times$W/4 \\
\#4 & ResidualBlock (x2)$\shortrightarrow$Packing & 3 & 1 & 128$\times$H/8$\times$W/8 \\
\#5 & ResidualBlock (x3)$\shortrightarrow$Packing & 3 & 1 & 256$\times$H/16$\times$W/16 \\
\#6 & ResidualBlock (x3)$\shortrightarrow$Packing & 3 & 1 & 512$\times$H/32$\times$W/32 \\
\midrule
\multicolumn{5}{c}{\textbf{Depth Decoder}} \\ \hline
\#7  & UpsampleBlock (\#5) & 3 & 1  & 512$\times$H/16$\times$W/16 \\
\#8  & UpsampleBlock (\#4) & 3 & 1  & 256$\times$H/8$\times$W/8 \\
\#9  & UpsampleBlock (\#3) & 3 & 1  & 128$\times$H/4$\times$W/4 \\
\#10  & UpsampleBlock (\#2) & 3 & 1  & 64$\times$H/2$\times$W/2 \\
\#11  & UpsampleBlock (\#1) & 3 & 1  & 64$\times$H$\times$W \\
\#12 & Conv2d $\shortrightarrow$ Sigmoid & 3 & 1 &   1$\times$H$\times$W \\
\bottomrule
\end{tabular}
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\resizebox{0.50\linewidth}{!}{
\subfloat[BTS \cite{lee2019big} (20 fps)]{
\begin{tabular}[b]{l|l|c|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\toprule
\multicolumn{5}{c}{\textbf{ResidualBlock (K, S)}} \\ 
\midrule
\#A & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & 1 & 1 &  \\
\#B & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & K & 1 &  \\
\#C & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & 1 & S &  \\
\toprule
\multicolumn{5}{c}{\textbf{UpsampleBlock}} \\ 
\midrule
\#D & UpsampleBlock (2x) & & &\\ 
\#E & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU  & 3 & 1 & \\
\toprule
\multicolumn{5}{c}{\textbf{Conv2dBlock}} \\ 
\midrule
\#F & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & 3 & 1 &  \\
\#G & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU & 1 & 1 &  \\
\toprule
\toprule
\#0 & Input RGB image & - & - & 3$\times$H$\times$W \\ 
\midrule
\multicolumn{5}{c}{\textbf{Encoder}} \\ \hline
\#1  & Conv2d$\shortrightarrow$BN$\shortrightarrow$ReLU   & 7 & 2 &  64$\times$H/2$\times$W/2 \\
\#2  & Max. Pooling                 & 3 & 2 &   64$\times$H/2$\times$W/2 \\
\#3  & ResidualBlock (x3)           & 3 & 2 &  256$\times$H/4$\times$W/4 \\
\#4  & ResidualBlock (x4)           & 3 & 2 &  512$\times$H/8$\times$W/8 \\
\midrule
\multicolumn{5}{c}{\textbf{Depth Decoder}} \\ 
\midrule
\#5  & ASPP (\#4)                                   & 3 & 1 & 512$\times$H/8$\times$W/8 \\
\#6  & Local Planar Guidance (\#5)                  & 3 & 1 & 512$\times$H$\times$W \\
\#7  & UpsampleBlock (\#5)                          & 3 & 1 & 256$\times$H/4$\times$W/4 \\
\#8  & Downsample (\#6)                             & 3 & 1 & 256$\times$H/4$\times$W/4 \\
\#9  & Conv2dBlock (\#3$\oplus$\#7$\oplus$\#8)  & 3 & 1 & 256$\times$H/4$\times$W/4 \\
\#10 & Local Planar Guidance (\#9)                  & 3 & 1 & 256$\times$H$\times$W \\
\#11 & UpsampleBlock (\#9)                          & 3 & 1 & 128$\times$H/2$\times$W/2 \\
\#12 & Downsample (\#10)                            & 3 & 1 & 128$\times$H/2$\times$W/2 \\
\#13 & Conv2dBlock (\#2$\oplus$\#11$\oplus$\#12)    & 3 & 1 & 128$\times$H/2$\times$W/2 \\
\#14 & Local Planar Guidance (\#15)                 & 3 & 1 & 128$\times$H$\times$W \\
\#15 & UpsampleBlock (\#16)                         & 3 & 1 &  64$\times$H$\times$W \\
\#16 & Reduction (\#17)                             & 3 & 1 &  32$\times$H$\times$W \\
\#17 & Conv2dBlock (\#6$\oplus$\#10$\oplus$\#14$\oplus$\#16) & 3 & 1 & 1$\times$H$\times$W \\
\#18 & Sigmoid (\#17) & & & 1$\times$H$\times$W \\
\bottomrule
\end{tabular}
}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{
\textbf{Different depth networks used in this work.} The depth network outputs $1 \times H \times W$ tensors with predicted inverse depth values, that are scaled between the minimum and maximum depth ranges. \emph{BN} stands for Batch Normalization \cite{ioffe2015batch}, \emph{GN} for Group Normalization \cite{WuH18}, \emph{Dropout} is described in \cite{dropout14}, \emph{Upsample} doubles spatial dimensions using bilinear interpolation, \emph{ReLU} are Rectified Linear Units and \emph{ELU} are Exponential Linear Units \cite{clevert2016fast}. The symbol $\oplus$ indicates feature concatenation. Inference times were calculated using a Titan V100 GPU and batch size of $1$.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{tab:networks}
\end{table*}


% \begin{tabularx}{0.5\textwidth}{X|l}
% \shortrightarrowprule
% asdfasdf
% \shortrightarrowprule
% \end{tabularx}

==> sections/supp_resnet.tex <==
\begin{table}[!h]
\small
\renewcommand{\arraystretch}{1.1}
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|l|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{Output Tensor Dim.} \\ 
\toprule
\#0 & Input RGB image & & 3$\times$H$\times$W \\ 
\midrule
\midrule
\multicolumn{4}{c}{\textbf{ResidualBlock}} \\ \hline
& Conv2d + BatchNorm + ReLU & 3 &  \\
& Conv2d + BatchNorm        & 3 &  \\
\midrule
\multicolumn{4}{c}{\textbf{Depth Encoder}} \\ \hline
\#1  & Conv2d (S2) + BatchNorm + ReLU & 7 &  64$\times$H/2$\times$W/2 \\
\#2  & Conv2d + BatchNorm + ReLU            & 3 &  64$\times$H/2$\times$W/2 \\
\#3  & ResidualBlock (\#2)  x2              & - &  64$\times$H/2$\times$W/2 \\
\#4  & Max. Pooling ($\times$1/2)          & 3 &  64$\times$H/4$\times$W/4 \\
\#5  & ResidualBlock (\#3 + \$2) x2         & - & 128$\times$H/4$\times$W/4 \\
\#6  & Max. Pooling ($\times$1/2)          & 3 & 128$\times$H/8$\times$W/8 \\
\#7  & ResidualBlock (\#4 + \#3) x2         & - & 256$\times$H/8$\times$W/8 \\
\#8  & Max. Pooling ($\times$1/2)          & 3 & 256$\times$H/16$\times$W/16 \\
\#9  & ResidualBlock (\#5 + \#4) x2         & - & 512$\times$H/16$\times$W/16 \\
\midrule
\multicolumn{4}{c}{\textbf{Depth Decoder}} \\ 
\midrule
\#10 & Conv2D + ELU (\#9)                                   & 3 & 128$\times$H/16$\times$W/16 \\
\#11 & Conv2D + Upsample (\#10)                             & 3 & 128$\times$H/8$\times$W/8  \\
\textbf{\#12} & Conv2D + Sigmoid                            & 3 & 1$\times$H/8$\times$W/8 \\
\#13 & Conv2D + ELU                                         & 3 & 64$\times$H/8$\times$W/8 \\
\#14 & Conv2D + Upsample(\#7 $\oplus$ \#13)                 & 3 & 64$\times$H/4$\times$W/4  \\
\textbf{\#15} & Conv2D + Sigmoid                            & 3 & 1$\times$H/8$\times$W/8 \\
\#16 & Conv2D + ELU                                         & 3 & 32$\times$H/4$\times$W/4 \\
\#17 & Conv2D + Upsample (\#5 $\oplus$ \#16)                & 3 & 32$\times$H/2$\times$W/2  \\
\textbf{\#18} & Conv2D + Sigmoid                            & 3 & 1$\times$H/8$\times$W/8 \\
\#19 & Conv2D + ELU                                         & 3 & 16$\times$H/2$\times$W/2 \\
\#20 & Conv2D + Upsample (\#3 $\oplus$ \#19)                & 3 & 16$\times$H$\times$W  \\
\textbf{\#21} & Conv2D + Sigmoid                            & 3 & 1$\times$H$\times$W \\
\bottomrule
\end{tabular}
% }
\caption{\textbf{ResNet architecture.} Line numbers in bold indicate output inverse depth layer scales. \emph{Upsample} is a nearest-neighbor interpolation operation that doubles the spatial dimensions of the input tensor. $\oplus$ denotes feature concatenation for skip connections.}
\label{table:supp-resnet-arch}
\end{table}

==> sections/supp_table_in_class.tex <==

% IN-CLASS GENERALIZATION (PACKNET)

\begin{table}[h!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{cc|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{In-Class Generalization (dotless dataset)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}}}
& \textbf{Method} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
&  & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

& PackNet~\cite{packnet} & 0.007 & 0.005 & 0.009 & 0.821 & 0.999 & 1.000 & 1.000  \\

& ResNet~\cite{he2016deep} & \textbf{0.005} & \textbf{0.004} & \textbf{0.007} & \textbf{0.677} & \textbf{1.000} & \textbf{1.000} & \textbf{1.000} \\

& BTS~\cite{lee2019big} & 0.010  & 0.007   &  0.013   & 1.189 & 0.998 & 1.000 & 1.000 \\

\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for in-class generalization, using different networks.}
\label{table:depth-in-class-dotless}
\end{table}



==> sections/table_depth_bts.tex <==

% CROSS-OBJECT GENERALIZATION (PACKNET)

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{PackNet: Cross-object generalization (dotted)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{LOO}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Mug}}}}

& \textit{Mug}
& 0.034 & 0.013 & 0.041 & 3.230 & 0.776 & 0.978 & 0.997 \\
& \textit{Box}
& 0.017 & 0.008 & 0.024 & 2.384 & 0.952 & 0.994 & 0.998 \\
& \textit{Glass}
& 0.016 & 0.008 & 0.023 & 2.328 & 0.954 & 0.994 & 0.999 \\
& \textit{Finger}
& 0.018 & 0.008 & 0.026 & 2.579 & 0.940 & 0.991 & 0.998 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Glass}}}}

& \textit{Mug}
& 0.017 & 0.008 & 0.024 & 2.380 & 0.952 & 0.995 & 0.999 \\
& \textit{Box}
& 0.017 & 0.008 & 0.024 & 2.378 & 0.952 & 0.994 & 0.999 \\
& \textit{Glass}
& 0.030 & 0.012 & 0.043 & 3.868 & 0.811 & 0.973 & 0.997 \\
& \textit{Finger}
& 0.018 & 0.008 & 0.026 & 2.572 & 0.940 & 0.991 & 0.998 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Finger}}}}

& \textit{Mug}
& 0.019 & 0.010 & 0.036 & 3.566 & 0.949 & 0.991 & 0.994 \\
& \textit{Box}
& 0.018 & 0.011 & 0.035 & 3.537 & 0.950 & 0.990 & 0.994 \\
& \textit{Glass}
& 0.018 & 0.010 & 0.035 & 3.478 & 0.952 & 0.990 & 0.994 \\
& \textit{Finger}
& 0.028 & 0.014 & 0.046 & 4.352 & 0.845 & 0.972 & 0.990 \\


\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Box}}}}

& \textit{Mug}
& 0.019 & 0.010 & 0.033 & 3.233 & 0.948 & 0.991 & 0.994 \\
& \textit{Box}
& 0.042 & 0.017 & 0.056 & 5.244 & 0.702 & 0.907 & 0.966 \\
& \textit{Glass}
& 0.018 & 0.010 & 0.032 & 3.193 & 0.949 & 0.990 & 0.994 \\
& \textit{Finger}
& 0.020 & 0.011 & 0.034 & 3.333 & 0.934 & 0.986 & 0.993 \\

\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (PackNet \cite{packnet}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-obj-dotted}
\end{table*}


% CROSS-OBJECT GENERALIZATION (BTS)

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{BTS: Cross-object generalization (dotted)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{LOO}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Mug}}}}

& \textit{Mug}
& 0.041 & 0.016 & 0.053 & 4.859 & 0.712 & 0.924 & 0.977 \\
& \textit{Box}
& 0.017 & 0.007 & 0.023 & 2.296 & 0.956 & 0.996 & 0.999 \\
& \textit{Glass}
& 0.016 & 0.007 & 0.023 & 2.249 & 0.959 & 0.996 & 0.999 \\
& \textit{Finger}
& 0.017 & 0.008 & 0.024 & 2.345 & 0.953 & 0.995 & 0.999 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Glass}}}}

& \textit{Mug}
& 0.017 & 0.008 & 0.024 & 2.292 & 0.954 & 0.996 & 0.999 \\
& \textit{Box}
& 0.017 & 0.008 & 0.024 & 2.305 & 0.953 & 0.995 & 0.999 \\
& \textit{Glass}
& 0.034 & 0.013 & 0.045 & 4.078 & 0.775 & 0.950 & 0.987 \\
& \textit{Finger}
& 0.018 & 0.008 & 0.024 & 2.353 & 0.949 & 0.995 & 0.999 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Finger}}}}

& \textit{Mug}
& 0.019 & 0.008 & 0.025 & 2.336 & 0.947 & 0.996 & 0.999 \\
& \textit{Box}
& 0.019 & 0.008 & 0.025 & 2.349 & 0.945 & 0.995 & 0.999 \\
& \textit{Glass}
& 0.019 & 0.008 & 0.025 & 2.295 & 0.949 & 0.995 & 0.999 \\
& \textit{Finger}
& 0.037 & 0.017 & 0.053 & 5.273 & 0.776 & 0.925 & 0.968 \\


\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Box}}}}

& \textit{Mug}
& 0.018 & 0.008 & 0.025 & 2.431 & 0.948 & 0.994 & 0.999\\
& \textit{Box}
& 0.043 & 0.017 & 0.056 & 5.273 & 0.721 & 0.882 & 0.952 \\
& \textit{Glass}
& 0.017 & 0.008 & 0.024 & 2.372 & 0.952 & 0.994 & 0.999 \\
& \textit{Finger}
& 0.018 & 0.008 & 0.025 & 2.475 & 0.945 & 0.993 & 0.999 \\

\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (BTS \cite{lee2019big}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-obj-dotted}
\end{table*}

% DOTLESS CROSS-OBJECT GENERALIZATION

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{PackNet: Cross-object generalization (dotless)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{LOO}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Glass}}}}

& \textit{Glass}
& 0.033 & 0.022 & 0.040 & 3.962 & 0.778 & 0.957 & 0.997 \\
& \textit{Box}
& 0.009 & 0.006 & 0.011 & 1.016 & 0.998 & 1.000 & 1.000 \\
& \textit{Finger}
& 0.010 & 0.008 & 0.014 & 1.325 & 0.992 & 0.999 & 1.000 \\

\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Box}}}}

& \textit{Glass}
& 0.008 & 0.007 & 0.012 & 1.206 & 0.994 & 0.999 & 0.999 \\
& \textit{Box}
& 0.030 & 0.021 & 0.038 & 3.193 & 0.791 & 0.971 & 0.999 \\
& \textit{Finger}
& 0.009 & 0.007 & 0.014 & 1.314 & 0.992 & 0.999 & 1.000 \\

\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{Finger}}}}

& \textit{Glass}
& 0.008 & 0.006 & 0.011 & 1.052 & 0.997 & 1.000 & 1.000 \\
& \textit{Box}
& 0.008 & 0.006 & 0.010 & 1.006 & 0.998 & 1.000 & 1.000 \\
& \textit{Finger}
& 0.037 & 0.027 & 0.048 & 4.562 & 0.723 & 0.910 & 0.975 \\


\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (PackNet \cite{packnet}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-obj-dotless}
\end{table*}

% CROSS-CAMERA GENERALIZATION

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|cccc|ccc}
\toprule
\multicolumn{9}{c}{\textbf{PackNet: Cross-camera generalization (dotted)}} \\
\toprule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{Cam}}}}
& \textbf{Evaluation} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& \textbf{Dataset} & 
Abs.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.05$ &
$\delta<1.05^2$ &
$\delta<1.05^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Left}}}}
& \textit{Mug}
& 0.032 & 0.013 & 0.042 & 3.926 & 0.785 & 0.974 & 0.996 \\
& \textit{Box}
& 0.053 & 0.023 & 0.067 & 5.434 & 0.532 & 0.844 & 0.961 \\
& \textit{Glass}
& 0.064 & 0.028 & 0.080 & 4.738 & 0.377 & 0.780 & 0.949 \\
& \textit{Finger}
& 0.062 & 0.025 & 0.076 & 6.157 & 0.430 & 0.806 & 0.945 \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Right}}}}

& \textit{Mug}
& 0.036 & 0.017 & 0.055 & 4.959 & 0.746 & 0.965 & 0.985 \\
& \textit{Box}
& 0.033 & 0.015 & 0.052 & 5.087 & 0.814 & 0.968 & 0.986 \\
& \textit{Glass}
& 0.048 & 0.021 & 0.068 & 6.246 & 0.602 & 0.918 & 0.974 \\
& \textit{Finger}
& 0.049 & 0.020 & 0.069 & 6.212 & 0.626 & 0.905 & 0.970 \\

\bottomrule

\end{tabular}
}
\caption{Monocular depth estimation results for dataset transfer (PackNet \cite{packnet}). Independent models were trained using input-output pairs from each of the considered datasets, and evaluated separately on all considered datasets.}
\label{tab:depth-cam-dotted}
\end{table*}




